How Robust are the Estimated Effects of Nonpharmaceutical Interventions against COVID-19?

To what extent are effectiveness estimates of nonpharmaceutical interventions (NPIs) against COVID-19 influenced by the assumptions our models make? To answer this question, we investigate 2 state-of-the-art NPI effectiveness models and propose 6 variants that make different structural assumptions. In particular, we investigate how well NPI effectiveness estimates generalise to unseen countries, and their sensitivity to unobserved factors. Models that account for noise in disease transmission compare favourably. We further evaluate how robust estimates are to different choices of epidemiological parameters and data. Focusing on models that assume transmission noise, we find that previously published results are remarkably robust across these variables. Finally, we mathematically ground the interpretation of NPI effectiveness estimates when certain common assumptions do not hold.

==> npi_table.tex <==
\begin{table}[ht]
    \caption{NPIs modelled}
    \label{Table:NPIs}
    \centering 
    %\setlength{\tabcolsep}{2pt}
    %\resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.19\textwidth}p{0.7\textwidth}}
    \hline
    \textbf{NPI} & \textbf{Criteria} 
    \\ \hline
    Mask-wearing & 
    {\small{Either a country has implemented a policy of requiring mask usage among the general public, or survey reports indicating that over 60\% of people were wearing masks in public.}}
    \\ \hline
    Symptomatic testing & 
    {\small{Testing available to those with symptoms (defined by the country).}} \\ \hline
    Gatherings $<1000$ & 
    {\small{A country has set a size limit on gatherings, below 1000.}}
    \\ \hline
    Gatherings $<100$ & 
    {\small{A country has set a size limit on gatherings, below 100.}} 
    \\ \hline
    Gatherings $< 10$ & 
    {\small{A country has set a size limit on gatherings, below 10.}} 
    \\ \hline
    Some businesses closed & 
    {\small{A country has specified customer-facing businesses (restaurants, bars, gyms) that are considered “high risk” and need to suspend operations (blacklist). By default, businesses are not suspended.}} 
    \\ \hline
    Most nonessential businesses closed & 
    {\small{A country has suspended the operations of many customer-facing businesses. Customer-facing businesses are suspended unless designated essential.}} 
    \\ \hline
    Schools closed & 
    {\small{A country has closed many or all schools. (Note that this was accompanied by closing universities in more than 75\% of cases in our data.)}} 
    \\ \hline
    Stay-at-home order (with exemptions) & 
    {\small{A mandatory order for the general public to stay at home has been issued, with necessary exemptions.}}
    \\ \hline
    \end{tabular}
\end{table}
